Timespot1: A 28nm CMOS Pixel Read-Out ASIC for 4D Tracking at High Rates

We present the first characterization results of Timespot1, an ASIC designed in CMOS 28 nm technology, featuring a $32 \times 32$ pixel matrix with a pitch of $55 ~ \mu m$. Timespot1 is the first small-size prototype, conceived to readout fine-pitch pixels with single-hit time resolution below $50 ~ ps_\text{rms}$ and input rates of several hundreds of kilohertz per pixel. Such experimental conditions will be typical of the next generation of high-luminosity collider experiments, from the LHC run5 and beyond. Each pixel of the ASIC includes a charge amplifier, a discriminator, and a Time-to-Digital Converter with time resolution indicatively of $22.6 ~ ps_\text{rms}$ and maximum readout rates (per pixel) of $3 ~ MHz$. To respect system-level constraints, the timing performance has been obtained keeping the power budget per pixel below $40 ~ \mu W$. The ASIC has been tested and characterised in the laboratory concerning its performance in terms of time resolution, power budget and sustainable rates. The ASIC will be hybridized on a matched $32 \times 32$ pixel sensor matrix and will be tested under laser beam and Minimum Ionizing Particles in the laboratory and at test beams. In this paper we present a description of the ASIC operation and the first results obtained from characterization tests concerning its performance.

==> appunti/tabReview_vecchia.tex <==
\newcommand{\tx}[0]{\relax\ifmmode \times \else $\times$\fi}
\newcommand{\ep}[1]{\relax\ifmmode \times 10^{#1} \else $\times 10^{#1}$\fi}
\newcommand{\na}[0]{n.a.\xspace}

\begin{table*}
\caption{State of art of Timing Front-End ASICs}
\label{table}
\setlength{\tabcolsep}{3pt}

\begin{tabular}{|p{54pt}|p{18pt}|p{18pt}p{28pt}p{36pt}p{30pt}p{30pt}p{30pt}p{30pt}p{30pt}p{30pt}p{34pt}p{30pt}p{32pt}|}
% per fare le linee verticali e decidere la spaziaturea \begin{tabular}{|p{25pt}|p{75pt}|p{115pt}|}
%linea orizonatle\hline
\hline
ASIC & year & node & Time Res & pixel size & \# of pixels & power per channel & power per unit area&  sensor type & input capacitance & MiP & Hit rate & TW correction & FoM \eqref{eq:fom} \\ 
\hline
 & & [\SI{}{\nano\meter}]& [\SI{}{\pico\second}] & [\SI{}{\micro \meter}] &  & [\SI{}{\micro\watt}]& [\SI{}{\watt / \centi \meter ^2}]& & [\SI{}{\femto\farad}] & \SI{}{\femto\coulomb} & \SI{}{\giga  Hits / \centi\meter^2} & &\\ 

\hline

\textbf{Timespot1}$^{\mathrm{ab}}$           & 2021 & 28  & 50   & 55\tx55  & 1024         & 40 & 1.32   & 3D-Si, 3D-Diam. & 15? & 1.8 & 99  & ToT & 1.53\ep{-2}\\

Timepix4$^{\mathrm{b}}$ \cite{bib:tpix_42022} & 2020 & 65  & 135  & 55\tx55 & \SI{229e3}{}  & 18   &0.60 &  & 45 & 1.6 & 500 oppure 0.36 ??? & ToT & 1.23\ep{-2}\\

FAST2 \cite{bib:fast2}     & 202? & 110  & 36  & 500\tx500 & 32          & \SI{3e3}{} & 1.2 & UFSD & \SI{3.4e3}{} & 16 & 120 & soft CFD & 2.31\ep{-2}\\

FastIC$^{\mathrm{c}}$\cite{bib:fastic} & 202? & 65 & 107 & 1500\tx1500 & 8 & 12\ep{3} & 0.53? & MCT, SiPM, PMT  & \na & \na & \na & ToT &1.76\ep{-2}\\

DIAMASIC\cite{bib:diamasic} & 202?  & 130 & 80  & \na & \na & 1.5\ep{3} & \na & Diamond Strip & 1\ep{3}  & 10 & \na & no&\\

TOFHIR2X \cite{bib:tofhir2x} & 2021  & 130   & 24 BoL, 55 EoL  & 3000\tx3000 & 32 & 12.4\ep{3} & 0.11 & SiPM & \na & \na & 2.8\ep{-2} & amplitude &6.99\ep{-2}\\

ETROC1$^{\mathrm{c}}$\cite{bib:etroc1} & 202? & 65  & 29  & 1300\tx 1300 & 16 & 2.37\ep{3} & 0.14 & LGAD  & 3.5\ep3 & 6 & 2.3 & ToT & 0.246\\

ALTIROC1\cite{bib:altiroc1} & 2020 & 130  &  35 BoL, 70 EoL & 1300\tx1300 & 25 & 4.4\ep{3}  & 0.26  & LGAD & 6\ep3 & 4 & \na & ToT &0.110\\

FASTPIX$^{\mathrm{c}}$\cite{bib:fastpix} & 2021 & 180  &  142  & 20 hex & 68 & \na & \na & monolithic  & 0.054? & \na & \na  & ToT &\\

FCFD0$^{\mathrm{bc}}$\cite{bib:fcfd0} & 2021 & 65 &  30 & \na  & 3 & \na & \na & LGAD & 3.4 & 5 & \na &CFD & \\

%Another &  &  &   & & & & &  & & & & &\\
\hline
\multicolumn{14}{p{500pt}}{The ASICs presented in this table features a time resolution better than \SI{200}{\pico\second} experimentally measured. The test have been performed with an actual sensor an radiation source or with an electrical auto-test.  In case results from auto-test the circuit input capacitance is presented; in case of test with sensor, the total capacitance at the input node is presented.   Data are flageed as \na when either not available or not applicable.}\\
\multicolumn{14}{p{200pt}}{$^{\mathrm{a}}$This work,$^{\mathrm{b}}$ Electrical auto-test only.,$^{\mathrm{c}}$no TDC}
\end{tabular}
\label{tab:review}
\end{table*}



==> appunti/timing_ASICs.tex <==
HVMAPS25	monlitico	10ns 	25x35u
FAST2		LGAD		30 ps	500x500
FastIC		SIPM		140ps 	?
DIAMASIC 	diamante 	80ps	1.27x1.27mu
SOFIST4		monlitico	?	20x20u poche info bassa res (540ns....)
TOFHIR2X	SIPM		30ps	?
ETROC1		LGAD		30ps	?
ALTIROC 	LGAD		25ps	1.3x1.3mm
SliT128B	strip		5ns	    ?   5ns ... non ne vale la pena
Timpix3		?		    1.6ns	55x55u
Timpix4		?           <200ps  55x55u
Fastpix     ?           142ps   20x20u (esagonale)
FCFD0?

==> tabReview.tex <==
\newcommand{\tx}[0]{\relax\ifmmode \times \else $\times$\fi}
\newcommand{\ep}[1]{\relax\ifmmode \times 10^{#1} \else $\times 10^{#1}$\fi}
\newcommand{\na}[0]{n.a.\xspace}

\begin{table}
\caption{State of art of Timing Front-End ASICs}
\label{tableState}
\setlength{\tabcolsep}{2pt}

\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{p{56pt}C{18pt}C{18pt}C{28pt}C{40pt}C{30pt}C{30pt}}
% per fare le linee verticali e decidere la spaziatura \begin{tabular}{|p{25pt}|p{75pt}|p{115pt}|}
%linea orizonatle\hline
\toprule
ASIC name & year & node & time res & pixel size & \# of & TW cor-  \\ 
 & & [\SI{}{\nano\meter}]& [\SI{}{\pico\second}] & [\SI{}{\micro \meter}] &  pixels   & rection \\ 

\midrule

\textbf{Timespot1}$^{\mathrm{ab}}$ & 2021 & 28  & 50   & 55\tx55  & 1024 & ToT \\

Timepix4$^{\mathrm{b}}$ \cite{bib:tpix_42022} & 2020 & 65  & 135  & 55\tx55 & \num{229e3}  & ToT \\
FASTPIX$^{\mathrm{c}}$\cite{bib:fastpix} & 2021 & 180  &  142  & 10 to 20 & 68 & ToT \\
FAST2 \cite{bib:fast2}     & 2021 & 110  & 36  & 500\tx500 & 32          & soft CFD \\
FastIC$^{\mathrm{c}}$\cite{bib:fastic} & 2021 & 65 & 107 & 1500\tx1500 & 8 & ToT \\
DIAMASIC\cite{bib:diamasic} & 2021  & 130 & 80  & \na & \na & no \\
TOFHIR2X \cite{bib:tofhir2x} & 2021  & 130   & 24 BoL, 55 EoL  & 3000\tx3000 & 32 & amplitude \\
ETROC1$^{\mathrm{c}}$\cite{bib:etroc1} & 2021 & 65  & 29  & 1300\tx 1300 & 16 & ToT \\
ALTIROC1\cite{bib:altiroc1} & 2020 & 130  &  35 BoL, 70 EoL & 1300\tx1300 & 25 & ToT \\
FCFD0$^{\mathrm{bc}}$\cite{bib:fcfd0} & 2021 & 65 &  30 & \na  & 3 & CFD  \\

%Another &  &  &   & & & & &  & & & & &\\
\bottomrule

\multicolumn{7}{p{\columnwidth}}{The ASICs presented in this table feature a measured time resolution better than \SI{200}{\pico\second}. Measurements have been performed with an actual sensor and radiation source or with an electrical auto-test. Data are flaged as \na when either not available or not applicable.}\\
\multicolumn{7}{p{200pt}}{$^{\mathrm{a}}$This work,$^{\mathrm{b}}$ Electrical auto-test only.,$^{\mathrm{c}}$no TDC}
\end{tabular}
\end{adjustbox}
\label{tab:review}
\end{table}


